Heavy-element Accretion by Proto-Jupiter in a Massive Planetesimal Disk, Revisited

Planetesimal accretion is a key source for heavy-element enrichment in giant planets. It has been suggested that Jupiter's enriched envelope is a result of planetesimal accretion during its growth assuming it formed in a massive planetesimal disk. In this study, we simulate Jupiter's formation in this scenario. We assume in-situ formation and perform N-body simulations to infer the solid accretion rate. We find that tens-Earth masses of planetesimals can be captured by proto-Jupiter during the rapid gas accretion phase. However, if several embryos are formed near Jupiter's core, which is an expected outcome in the case of a massive planetesimal disk, scattering from the embryos increases the eccentricity and inclination of planetesimals and therefore significantly reduces the accretion efficiency. We also compare our results with published semi-analytical models and show that these models cannot reproduce the N-body simulations especially when the planetesimal disk has a large eccentricity and inclination. We show that when the dynamical evolution of planetesimals is carefully modelled, the total mass of captured planetesimals $M_\mathrm{cap,tot}$ is $2 M_\oplus \lesssim M_\mathrm{cap,tot}\lesssim 18 M_\oplus$. The metallicity of Jupiter's envelope can be explained by the planetesimal accretion in our massive disk model despite the low accretion efficiency coming from the high eccentricity and inclination of planetesimals. Our study demonstrates the importance of detailed modelling of planetesimal accretion during the planetary growth and its implications to the heavy-element mass in gaseous planets.

==> Planetesimal Accretion in Massive Planetesimal Disk/newcommands.tex <==
\newcommand{\ikoma}[1]{\textcolor{red}{{\bf #1}}}
\newcommand{\ikome}[1]{\textcolor{magenta}{(\bf #1)}}
\newcommand{\shibata}[1]{\textcolor[rgb]{0,0.5,0}{\bf #1}}
\newcommand{\remove}{\textcolor[gray]{0.8}}

%-------------------------------------
% Abbreviation
\newcommand{\rom}[1]{\MakeUppercase{\romannumeral #1}} %Roman number
\newcommand{\Mcrsb}{M_{\rm oc}^{\rm cr(sb)}}
\newcommand{\comsb}{COM-SB}
\newcommand{\comhp}{COM-HP}

%-------------------------------------
% Units
\newcommand{\g}{{\rm g}}
\newcommand{\kg}{{\rm kg}}
\newcommand{\cm}{{\rm cm}}
\newcommand{\m}{{\rm m}}
\newcommand{\km}{{\rm km}}
\newcommand{\AU}{{\rm ~au}}

\newcommand{\K}{{\rm K}}
\newcommand{\yr}{{\rm yr}}
\newcommand{\yrs}{{\rm yrs}}

%-------------------------------------
% Physical Parameters
\newcommand{\Gconst}{G}

\newcommand{\Msun}{M_{\odot}}
\newcommand{\Mjup}{M_{\rm Jup}}
\newcommand{\Mear}{M_{\oplus}}
\newcommand{\Rjup}{R_{\rm Jup}}



